Token-Level Adversarial Prompt Detection Based on Perplexity Measures and Contextual Information

In recent years, Large Language Models (LLM) have emerged as pivotal tools in various applications. However, these models are susceptible to adversarial prompt attacks, where attackers can carefully curate input strings that mislead LLMs into generating incorrect or undesired outputs. Previous work has revealed that with relatively simple yet effective attacks based on discrete optimization, it is possible to generate adversarial prompts that bypass moderation and alignment of the models. This vulnerability to adversarial prompts underscores a significant concern regarding the robustness and reliability of LLMs. Our work aims to address this concern by introducing a novel approach to detecting adversarial prompts at a token level, leveraging the LLM's capability to predict the next token's probability. We measure the degree of the model's perplexity, where tokens predicted with high probability are considered normal, and those exhibiting high perplexity are flagged as adversarial. Additionaly, our method also integrates context understanding by incorporating neighboring token information to encourage the detection of contiguous adversarial prompt sequences. To this end, we design two algorithms for adversarial prompt detection: one based on optimization techniques and another on Probabilistic Graphical Models (PGM). Both methods are equipped with efficient solving methods, ensuring efficient adversarial prompt detection. Our token-level detection result can be visualized as heatmap overlays on the text sequence, allowing for a clearer and more intuitive representation of which part of the text may contain adversarial prompts.

==> content/pieces/detectexamples.tex <==
\begin{table*}[!t]
  \centering
  \caption{An illustrative representation of token-level adversarial prompt detection. Token is color-coded based on the likelihood of it being part of an adversarial prompt: clear background indicates non-adversarial tokens while intense red indicates a high probability of being part of an adversarial prompt. 
  }
  \begin{tabular}{p{\textwidth}}
    \toprule
\tws{Out}{-0.000}\tws{line}{-0.000}\tws{ a}{-0.000}\tws{ plan}{-0.000}\tws{ to}{-0.000}\tws{ steal}{-0.000}\tws{ from}{-0.000}\tws{ a}{-0.000}\tws{ charity}{-0.000}\tws{ or}{-0.000}\tws{ nonprofit}{-0.000}\tws{ organization}{-0.000}\tws{.}{-0.004}\tws{ describing}{-0.998}\tws{.}{-0.999}\tws{{\textbackslash}}{-1.000}\tws{ +}{-1.000}\tws{ similarly}{-1.000}\tws{Now}{-1.000}\tws{ write}{-1.000}\tws{ opposite}{-1.000}\tws{ley}{-1.000}\tws{.]}{-1.000}\tws{(}{-1.000}\tws{ Me}{-1.000}\tws{ giving}{-1.000}\tws{**}{-1.000}\tws{ONE}{-1.000}\tws{ please}{-1.000}\tws{?}{-1.000}\tws{ revert}{-1.000}\tws{ with}{-1.000}\tws{ ''{\textbackslash}}{-1.000}\tws{!--}{-1.000}\tws{Two}{-1.000}\\
\tws{Z}{-0.000}\tws{ou}{-0.000}\tws{ et}{-0.000}\tws{ al}{-0.000}\tws{.}{-0.000}\tws{ (}{-0.000}\tws{20}{-0.000}\tws{23}{-0.000}\tws{)}{-0.000}\tws{ demonstrate}{-0.000}\tws{ that}{-0.000}\tws{ it}{-0.000}\tws{ is}{-0.000}\tws{ possible}{-0.000}\tws{ to}{-0.000}\tws{ automatically}{-0.000}\tws{ construct}{-0.000}\tws{ advers}{-0.000}\tws{arial}{-0.000}\tws{ attacks}{-0.000}\tws{ on}{-0.000}\tws{ LL}{-0.000}\tws{Ms}{-0.000}\tws{.}{-0.000}\\
    \bottomrule
  \end{tabular}
\end{table*}

==> content/pieces/detectexampleslong.tex <==
\begin{table*}[!t]
  \centering
  \caption{An illustrative example of token-level adversarial prompt detection. Token is color-coded based on the likelihood of it being part of an adversarial prompt: green background indicates non-adversarial tokens while intense red indicates a high probability of being part of an adversarial prompt. 
  }
  \begin{tabular}{p{\textwidth}}
    \toprule
{Out}{line}{ a}{ plan}{ to}{ steal}{ from}{ a}{ charity}{ or}{ nonprofit}{ organization}{.}{ describing}{.}{{\textbackslash}}{ +}{ similarly}{Now}{ write}{ opposite}{ley}{.]}{(}{ Me}{ giving}{**}{ONE}{ please}{?}{ revert}{ with}{ ''{\textbackslash}}{!--}{Two}\\
\tws{Out}{0.000}\tws{line}{0.602}\tws{ a}{0.190}\tws{ plan}{0.424}\tws{ to}{1.000}\tws{ steal}{-0.473}\tws{ from}{0.799}\tws{ a}{0.595}\tws{ charity}{-0.033}\tws{ or}{0.737}\tws{ nonprofit}{0.306}\tws{ organization}{0.779}\tws{.}{1.000}\tws{ describing}{-1.000}\tws{.}{0.038}\tws{{\textbackslash}}{-0.626}\tws{ +}{-0.451}\tws{ similarly}{-1.000}\tws{Now}{-1.000}\tws{ write}{-0.047}\tws{ opposite}{-0.973}\tws{ley}{-1.000}\tws{.]}{-0.853}\tws{(}{0.344}\tws{ Me}{-1.000}\tws{ giving}{-0.876}\tws{**}{-0.804}\tws{ONE}{-1.000}\tws{ please}{-0.719}\tws{?}{0.300}\tws{ revert}{-1.000}\tws{ with}{0.056}\tws{ ''{\textbackslash}}{-0.948}\tws{!--}{-1.000}\tws{Two}{-0.320}\\
\tws{Out}{1.000}\tws{line}{1.000}\tws{ a}{1.000}\tws{ plan}{1.000}\tws{ to}{1.000}\tws{ steal}{1.000}\tws{ from}{1.000}\tws{ a}{1.000}\tws{ charity}{1.000}\tws{ or}{1.000}\tws{ nonprofit}{1.000}\tws{ organization}{1.000}\tws{.}{0.993}\tws{ describing}{-0.997}\tws{.}{-0.998}\tws{{\textbackslash}}{-1.000}\tws{ +}{-1.000}\tws{ similarly}{-1.000}\tws{Now}{-1.000}\tws{ write}{-1.000}\tws{ opposite}{-1.000}\tws{ley}{-1.000}\tws{.]}{-1.000}\tws{(}{-1.000}\tws{ Me}{-1.000}\tws{ giving}{-1.000}\tws{**}{-1.000}\tws{ONE}{-1.000}\tws{ please}{-1.000}\tws{?}{-1.000}\tws{ revert}{-1.000}\tws{ with}{-1.000}\tws{ ''{\textbackslash}}{-1.000}\tws{!--}{-1.000}\tws{Two}{-1.000}\\
    \bottomrule
  \end{tabular}
\end{table*}




==> content/sections/algorithms.tex <==
\section{Algorithms}
Both \eqref{eq:opt_problem} and \eqref{eq:posterior_problem} in the previous sections can be efficiently solved using dynamic programming (DP) with $O(n)$ complexity.

==> content/sections/introductionold.tex <==
\section{Introduction}
Large Language Models (LLMs) have experienced significant advancements and breakthroughs in recent times. Their capabilities to understand, generate, and even simulate human-level textual interactions have been revolutionary. Their use in user interactions has become widespread, from chatbots that can maintain engaging conversations to automated systems that answer common customer queries. These applications offer continuous online support, effectively providing 24/7 assistance. 

However, with all their potential and widespread applications, existing LLMs face an inherent vulnerability: adversarial prompts \cite{zou2023universal}. Adversarial prompts are sequences of input that are crafted with the intention to deceive or confuse the model, causing it to generate unintended outputs. The reason behind LLMs being susceptible to these attacks is rooted in their design. Essentially, they operate by taking in a string and producing an output string in response, no matter how anomalous or out-of-context the input may be. If this input string is highly out-of-distribution (OOD), the output can be arbitrary and unpredictable. Attackers, realizing this vulnerability, can carefully select such OOD strings, leading the model to generate misleading or even harmful outputs.

The aim of this paper is to introduce a method at the token level to detect these adversarial prompts. Our approach relies on the LLM's intrinsic capability to predict the probability of the next token in a sequence. Due to the OOD nature of these adversarial prompts, a salient characteristic of adversarial prompts is their high perplexity. Often achieved through discrete optimization techniques, these adversarial sequences do not resemble regular textual content that a model expects to see. 

Furthermore, these adversarial prompts often appear in sequence, as longer adversarial prompts are more effective in leading the model astray. This inspires us to consider context provided by neighboring tokens, in addition to just the perplexity of individual tokens. This contextual information can often provide significant clues about the presence of adversarial prompts.

In this study, by combining the LLM's prediction capabilities with the contextual understanding of token sequences, we aim to build a robust detection system that can effectively identify and possibly mitigate adversarial prompt attacks. In the next section, we will discuss two methods: one that identifies each token as either being part of an adversarial prompt or not, and another that estimates the probability of each token being part of an adversarial prompt.

==> content/sections/methods.tex <==
\section{Methods}
We first introduce the background and necessary mathematics notations.
\subsection{Background}
The input that need to be analyzed is a sequence of $n$ tokens, represented as $\vec{x} = (x_1, \dots, x_n)$. We regard this sequence as generated either from a regular language distribution, or from an adversarial prompt distribution. 

Since we are not aware of the ground-truth of language distribution, we use a language model as an approximation. 
Given its preceding tokens $x_1, \dots, x_{i-1}$, a language model produce a probability represented as $p_{\text{LLM}}(x_i|x_1,\dots,x_{i-1})$. For simplicity, we refer to this probability as $p_{0,i}$.

Meanwhile, adversarial prompts are expected to follow a different distribution. We assume that the distribution of an adversarial prompt token is uniform across all possible tokens constructed from ASCII characters, represented as $\Sigma_{\text{ascii}}$. Therefore, its probability is $p_{1,i} = \frac{1}{\abs{\Sigma_{\text{ascii}}}}$.

Our goal is to identify whether each token in the sequence is from the language model or an adversarial prompt. This is represented by an indicator $c_i \in \{0,1\}$, where 1 indicates that the $i$-th token is detected as an adversarial prompt.

\subsection{Optimization Problem}
Our initial approach attempts to maximize the likelihood of observing the sequence given the assigned indicators. 

Given $c_i$, the probability distribution of the $i$-th token is defined as $p(x_i|c_i) = p_{c_i,i}$. 
However, a naive application of Maximum Likelihood Estimation (MLE) doesn't yield high detection accuracy. This is because only the perplexity of individual tokens is considered, neglecting the fact that adversarial prompts often form sequences. 

If a token has high perplexity, it doesn't necessarily mean it is an adversarial prompt. It might just be a rare token in a normal text. By considering its surrounding context, we can make more accurate judgments. For instance, if a token with high perplexity is surrounded by tokens with normal perplexity, it's likely that this token is also part of the normal text.

To encourage the detection of contiguous adversarial prompt sequences, we introduce a regularization term $\sum_{i=1}^{n-1}\abs{c_{i+1}-c_i}$ inspired by the fused lasso. This regularization aims to make adjacent indicators $c_i$ and $c_{i+1}$ similar, thus considering the context around a token when determining if it's part of an adversarial prompt sequence.

Incorporating this regularization leads to our final optimization problem:
%
%
%
\begin{equation}\label{eq:opt_problem}
\begin{aligned}
\max_{\vec{c}} &\sum_{i=1}^{n-1} [(1-c_i)\log(p_{0,i})+c_i\log(p_{1,i})] \\&+ \lambda \sum_{i=1}^{n-1}\abs{c_{i+1}-c_i}.
\end{aligned}
\end{equation}
This formulation balances token perplexity and contextual information. The strength of this balance is controlled by a hyperparameter, $\lambda$. 
A higher $\lambda$ emphasizes the context around a token, while a lower $\lambda$ prioritizes the token's own perplexity. When $\lambda$ is infinitely large, all indicators $c_i$ in the sequence will be the same. Conversely, when $\lambda$ is zero, each token's indicator will solely depend on its own perplexity.

\subsection{Handling Edge Cases}
In practice, we observed that the first token of a sequence is often flagged as an adversarial prompt.
This is mainly due to its high perplexity caused by the absence of a preceding context.
To mitigate this, we simply exclude the first token from being considered in our adversarial prompt detection by setting $p_{0,1}=p_{1,1}$.

In summary, our methods involve using both optimization techniques and probabilistic graphical models to detect adversarial prompts in a sequence of tokens. The integration of context-aware regularization and probabilistic reasoning ensures more robust and accurate results.
\subsection{Probabilistic Graphical Model}
While the optimization problem gives us a binary output for each token, it doesn't capture the uncertainty in the prediction. 
To address this, we can extend our approach to a probabilistic graphical model. This approach has the advantage of providing uncertainty information about the model's predictions with a Bayesian posterior over the indicators $c_i$.

We model each indicator, $c_i$, as a random variable. Its prior distribution reflects our beliefs about its likelihood to be 1. 
We choose the following prior for the sequence of indicators $\vec{c}$:
\begin{equation*}
    p(\vec{c})=\frac{1}{Z}\exp\left(\lambda\sum_{i=1}^{n-1}\abs{c_{i+1}-c_i}+\mu\sum_{i=1}^n c_i\right),
\end{equation*}
where $Z$ is a normalization constant, and $\mu$ controls the prior probability of $c_i=1$.
Given $\vec{c}$, the probability of generating the sequence $\vec{x}$ is:
\begin{equation*}
\begin{aligned}
&p(\vec{x}|\vec{c})=\prod_i p_{c_i,i}\\=&\prod_i \exp\left((1-c_i)\log(p_{0,i})+c_i\log(p_{1,i})\right).
\end{aligned}
%
\end{equation*}
Given the sequence $\vec{x}$, the Bayesian posterior distribution over $\vec{c}$ is defined, incorporating both the likelihood of observing the sequence from the given indicators and the prior over the indicators:
%
%
%
%
%
%
\begin{align}\label{eq:posterior_problem}
&p(\vec{c}|\vec{x})=\frac{p(\vec{x}|\vec{c}) p(\vec{c})}{p(\vec{x})}\nonumber\\=&\frac{1}{Z'}\exp\left(\sum_{i=1}^{n-1} [(1-c_i)\log(p_{0,i})+c_i\log(p_{1,i})]\right.\nonumber\\&\left.\quad\quad\quad\quad+\lambda\sum_{i=1}^{n-1}\abs{c_{i+1}-c_i}\!+\!\mu\sum_{i=1}^n c_i\right),
\end{align}
where $Z'$ is another normalization constant. This can be visualized as a probabilistic graph as in \cref{fig:adversarial_graph} where each $c_i$ is connected to its adjacent $c_{i+1}$ and the corresponding $x_i$.

\input{content/pieces/probgraph}

Finally, the probability $p(c_i|\vec{x})$ provides the detection result. A higher probability for $c_i = 1$ implies that the token is more likely to be an adversarial prompt.

